A Generalized Quantifier Concept in Computational Complexity Theory

A notion of generalized quantifier in computational complexity theory is explored and used to give a unified treatment of leaf language definability, oracle separations, type 2 operators, and circuits with monoidal gates. Relations to Lindstroem quantifiers are pointed out.

==> macros2e97.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% Sectioning
% 



% sections:
% 

\makeatletter
\renewcommand{\section}{\@startsection
	{section}%
	{1}%
	{0mm}%
	{-2\baselineskip}%
	{\baselineskip}%
	{\normalfont\large\bf}}
\renewcommand{\subsection}{\@startsection
	{subsection}%
	{1}%
	{0mm}%
	{-2\baselineskip}%
	{\baselineskip}%
	{\normalfont\normalsize\bf}}
\makeatother
	


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% Theorem environments and the like

% diverse layout changes
\makeatletter
\def\@begintheorem#1#2{\parskip0pt plus3pt\it \trivlist \item[\hskip 
\labelsep{\bf #1\ #2.}]}
\def\@opargbegintheorem#1#2#3{\parskip0pt plus3pt\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]}
\makeatother


% Environments with Text in Roman
% i.e.: Definitions

\makeatletter

\def\newdefinition#1{\@ifnextchar[{\@odefi{#1}}{\@ndefi{#1}}}

\def\@ndefi#1#2{%
\@ifnextchar[{\@xndefi{#1}{#2}}{\@yndefi{#1}{#2}}}

\def\@xndefi#1#2[#3]{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}\@addtoreset{#1}{#3}%
\expandafter\xdef\csname the#1\endcsname{\expandafter\noexpand
  \csname the#3\endcsname \@deficountersep \@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@yndefi#1#2{\expandafter\@ifdefinable\csname #1\endcsname
{\@definecounter{#1}%
\expandafter\xdef\csname the#1\endcsname{\@deficounter{#1}}%
\global\@namedef{#1}{\@defi{#1}{#2}}\global\@namedef{end#1}{\@enddefi}}}

\def\@odefi#1[#2]#3{\expandafter\@ifdefinable\csname #1\endcsname
  {\global\@namedef{the#1}{\@nameuse{the#2}}%
\global\@namedef{#1}{\@defi{#2}{#3}}%
\global\@namedef{end#1}{\@enddefi}}}

\def\@defi#1#2{\refstepcounter
    {#1}\@ifnextchar[{\@ydefi{#1}{#2}}{\@xdefi{#1}{#2}}}

\def\@xdefi#1#2{\@begindefi{#2}{\csname the#1\endcsname}\ignorespaces}
\def\@ydefi#1#2[#3]{\@opargbegindefi{#2}{\csname
       the#1\endcsname}{#3}\ignorespaces}

\def\@deficounter#1{\noexpand\arabic{#1}}
\def\@deficountersep{.}
%deleted September 2, 1986 MDK
%\def\@makethmnumber#1#2{\bf #1 #2:}
\def\@begindefi#1#2{\it \trivlist \item[\hskip \labelsep{\bf #1\ #2.}]\rm}
\def\@opargbegindefi#1#2#3{\it \trivlist
      \item[\hskip \labelsep{\bf #1\ #2\ #3.}]\rm}
\def\@enddefi{\endtrivlist}

\makeatother


%
% Environment-Vereinbarungen:

\newtheorem{thm}{Theorem}[section]
\newtheorem{coro}[thm]{Corollary}
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{propo}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}

\newtheorem{question}{Open Question}

\newdefinition{defi}[thm]{Definition}
\newdefinition{example}[thm]{Example}
\newdefinition{problem}[thm]{Problem}
\newdefinition{remark}[thm]{Remark}

% proof environment
\newcommand\qedsymbol{\ding{113}}
\def\endproof{{\unskip\nobreak\hfil\penalty50
		      \hskip1em\hbox{}\nobreak\qedsymbol
		      \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}} 
\def\proof{\trivlist
	\penum=1%penum: siehe unten!
	\item[\hskip \labelsep{\it Proof.}]}

\def\endoutline{{\unskip\nobreak\hfil\penalty50
		      \hskip1em\hbox{}\nobreak\qedsymbol
		      \parfillskip=0pt\par\endtrivlist\addpenalty{-100}}} 
\def\outline{\trivlist
	\penum=1%penum: siehe unten!
	\item[\hskip \labelsep{\it Proof sketch.}]}

% eigenes enumerate fuer Beweise, um Platz zu sparen ...
\newcount\penum
\def\pitem{\ifnum\penum>1\par\fi\the\penum. \advance\penum by1}


% numerierte Gleichungen, Bemerkungen, etc; 
% nur mit Nummer, ohne "Satz", "Korollar", ...

\newenvironment{eqn}
	{\trivlist\refstepcounter{thm}\item[\hskip \labelsep{\bf \thethm.}]}
	{\endtrivlist}



\newcounter{noheadsectionctr}[section]
\def\noheadsection{\addtocounter{noheadsectionctr}{1}
	\par\noindent{\bf\arabic{section}.\arabic{noheadsectionctr}. }}



\newcommand\todo[1]{\par{\sl #1}}
\newcommand\marg[1]{\marginpar{\raggedright\footnotesize\sl #1}}



